A Versatile Crack Inspection Portable System based on Classifier Ensemble and Controlled Illumination

This paper presents a novel setup for automatic visual inspection of cracks in ceramic tile as well as studies the effect of various classifiers and height-varying illumination conditions for this task. The intuition behind this setup is that cracks can be better visualized under specific lighting conditions than others. Our setup, which is designed for field work with constraints in its maximum dimensions, can acquire images for crack detection with multiple lighting conditions using the illumination sources placed at multiple heights. Crack detection is then performed by classifying patches extracted from the acquired images in a sliding window fashion. We study the effect of lights placed at various heights by training classifiers both on customized as well as state-of-the-art architectures and evaluate their performance both at patch-level and image-level, demonstrating the effectiveness of our setup. More importantly, ours is the first study that demonstrates how height-varying illumination conditions can affect crack detection with the use of existing state-of-the-art classifiers. We provide an insight about the illumination conditions that can help in improving crack detection in a challenging real-world industrial environment.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> sections/rebuttal.tex <==
\section*{\textbf{AUTHORS' RESPONSE FOR PAPER 1127}}
\noindent\textbf{\textit{A Versatile Crack Inspection Portable System based on Classifier Ensemble and Controlled Illumination}}
\subsection{\textbf{Response to Area Chair's comments}}
\noindent \textit{``This paper received a very convincing review recommending weak reject and suggesting a resubmission to the second round after revision. The review includes important points which should be addressed for the second round review to make this paper fit for acceptance. The authors are encouraged to make use of this second round process.''}

\noindent Dear Area Chair, we are thankful for the constructive comments given by both the reviewers. These comments were truly helpful in revising and improving the draft. We have now prepared the new submission based on the reviewer's comments and we here provide a point-by-point response to the reviewer's comments. Our response to the reviewers' comments is shown in \textcolor{blue}{blue color} and the words and sentences modified in the manuscript are shown in \changemarker{green color}.

\subsection{\textbf{Response to Comments of Reviewer \#1 (ID: 6297)}}

\noindent \textcolor{blue}{Thank you for your constructive comments and helpful suggestions.
%Apart from the modifications suggested by your comments, the revised paper also includes updated contents suggested by Reviewer\#2.
Below are the updates in the paper addressing your valuable suggestions.}
\newline

\noindent \textbf{1.} \textit{``This paper proposed the system and the method for crack inspection. For controlling the light conditions, the authors developed the illumination frame as shown in Figure 1 (a). The system uses patch-based recognition, where images are divided into several small patches and each patch is inputted to the DNN-based classifier. The authors investigated the performance of the various networks, such as pre-trained networks and two original networks that were shown in Figure 3.''}
\newline \noindent \textcolor{blue}{Thank you for summarizing our work. We indeed propose a novel setup for crack detection to address a real industrial inspection problem. Additionally, we also provide a unqiue study that demonstrates how lights placed at different heights can affect crack detection using the state-of-the-art classifiers, in a challenging industrial scenario. In order to clearly point out this novelty, we have included the following lines in the abstract.}
\changemarker{More importantly, ours is the first study that demonstrates how height-varying illumination conditions can affect crack detection with the use of existing state-of-the-art classifiers. We provide an insight about the illumination conditions that can help in improving crack detection in a challenging real-world industrial environment.}
% \changemarker{\textit{More importantly, to our best knowledge ours is the first of its kind of study that addresses height-varying illumination conditions in combination with existing deep learning classifiers; in order to provide a state-of-the-art solution for an automated crack detection problem in a challenging real-world industrial environment.}}
\newline

\noindent \textbf{2.} \textit{``I could not understand the conclusion of the paper. Is the conclusion that Xception\_finetune\_all achieves better performance in all the case? If so, what is the originality of the proposed method? The Xception\_finetune\_all has already proposed by the other group.''}
\newline
\noindent \textcolor{blue}{The original conclusion is about the different illumination conditions and their corresponding effect on crack detection. We demonstrate these using evaluation performed on classifiers trained with the state-of-the-art as well as our customized architectures. Importantly, our study suggests that lights placed at greater heights are more effective as compared to those placed near the tile’s surface for crack detection.}

\textcolor{blue}{Secondly, we acknowledge Xception to be one of the state-of-the-art architectures and we do not claim it to be the novelty of our work. Nevertheless, ours is the first study involving height-varying illumination conditions for crack detection and, therefore, it is also important to document how the existing state-of-the-art architectures have performed under these conditions. In this regard, our conclusions indicate Xception\_finetune\_all to be the best performing one across all the illumination conditions.}

\textcolor{blue}{Lastly, we also indicate how the crack detection performance is affected with the use of patches having different resolutions. The intuition of performance improvement with the use of high-resolution patches is validated in our study across all the lighting conditions. This should help in deciding the resolution versus performance trade-off for designing a real-time crack detection system for field use.}

\textcolor{blue}{We have now included the following in the revised conclusion.}
\changemarker{Our unique study on height-varying illumination conditions for crack detection suggests that lights placed at greater heights are more effective in detecting cracks as compared to those placed near the tile's surface. Our study also indicates that fine-tuning of all the pre-trained weights of the Xception architecture provide the best results in comparison to all the other trained models across all the illumination condition. Moreover, use of high-resolution patches (i.e., without downsampling the acquired images) for training further improves the results. Thus, the intuition of performance improvement with the use of high-resolution patches is also validated across all the lighting conditions in our study. This should help in deciding the resolution versus performance trade-off when designing a real-time crack detection system for field use. The effectiveness of different illumination conditions on crack detection has been demonstrated using evaluation performed on classifiers trained with the state-of-the-art as well as our customized architectures.}
%\changemarker{This evaluation has been performed using the existing state-of-the-art classification architectures as well as our customized architectures to have an unbiased and generalized observation. Being a novel study on height-varying illumination conditions, we also report the performance of the different architectures in these conditions. Our study indicates that fine-tuning of all the pre-trained weights of the Xception architecture provides the best results in comparison to all the other trained models across all the illumination condition. Moreover, use of high-resolution patches (i.e., without downsampling the acquired images) for training further improves the results. Thus, the intuition of performance improvement with the use of high-resolution patches is also validated across all the lighting conditions in our study. This should help in deciding the resolution versus performance trade-off when designing a real-time crack detection system for field use.}
\newline 

\noindent \textbf{3.} \textit{``Though the authors show the performance by the graph, it is better to show the actual value of the performance.''}
\newline
\noindent \textcolor{blue}{Thank you for this suggestion. We did present the numerical values for the performance of all the models in all the illumination conditions in a tabular form. However, reporting a large number of experimental results in a limited space using a tabular form made it extremely cluttered and confusing. We, therefore, used graphs to represent the results. Nevertheless, we did provide the numerical values for the best performing models in section \colorbox{green}{\ref{subsec:discussion_only}}, wherein we have now also included the numerical values for ${CCF1}$ score.}
\newline \newline 
\noindent \textbf{4.} \textit{``In pp 3, the authors distinguish negative, ambiguous, and positive patches using thresholds. Why did you choose 0.1 and 0.2 for the thresholds?''}
\newline
\noindent \changemarker{Intuitively, only those patches that contain no crack pixels (i.e., ${p = 0.0}$) should be labelled negative. Thus, setting ${p = 0.0}$ should suffice in labelling the patches as either negative or positive. However, in practice, the annotations are a few pixels wider than the actual crack-width, due to which some patches are incorrectly labelled as positive. To correctly label such patches as negative, we set a lower threshold to 0.1. Secondly, patches along the crack boundaries that contain few crack pixels have a similar appearance to that of the negative patches. Such ambiguous patches increase the number of false positives when labelled as positive. To avoid this, we set a higher threshold to 0.2.}
% \noindent \textcolor{blue}{The threshold 0.2 for positive patches was chosen heuristically based on the patch size and the minimum proportion of crack pixels that were generally observed in patches representing cracks. On the other hand, patches with a proportion of crack pixels less than 0.1 did not truly represent cracks. Therefore, these patches were labeled negative. Use of patches with crack pixel proportion between 0.1 and 0.2 as either positive or negative adversely affected the training and therefore these were considered ambiguous.}

% \textcolor{blue}{Thank you for pointing it out. We have now included the following line in section \ref{subsec:acquisition_and_registration} to clarify this.} \changemarker{The above thresholds are chosen heuristically based on patch size and observed proportion of annotated pixels in the crack and non-crack patches.}
\textcolor{blue}{Thank you for pointing it out. We have now included the above explanation in section \ref{subsec:acquisition_and_registration}.}
\newline \newline
\noindent \textbf{5.} \textit{``The proposed method solved the issue of imbalanced data by only using the data that are sampled with balancing for training. There are many ways for tackling the imbalance-data issue, such as: 
S. Wang, W. Liu, J. Wu, L. Cao, Q. Meng, and P. J. Kennedy, "Training deep neural networks on imbalanced data sets," 2016 International Joint Conference on Neural Networks (IJCNN), Vancouver, BC, 2016, pp. 4368-4374, doi: 10.1109/IJCNN.2016.7727770.''}
\newline
\noindent \textcolor{blue}{Thank you for this suggestion. Our data consists of few positive patches compared to a large number of negative patches per tile. The positive samples provide important features for crack detection while the negative samples have mostly repetitive non-crack information. For such data, i.e., where the minority class is of interest, balancing the training data with random under-sampling has been considered as one of the effective and widely accepted methods \cite{Buda_NN_2018}. The suggested reference \cite{Wang_IJCNN_2016} also mentions random under-sampling to be an easy and effective method, with the only problem that some features may be lost. This problem is automatically avoided in our case because training is performed using all the positive patches having the interesting crack-features while random sampling is done only for the negative patches.}

\textcolor{blue}{Use of a cost sensitive loss function as proposed in \cite{Wang_IJCNN_2016} is an alternative method to handle the problem of an imbalanced dataset. To verify this, we have retrained the Xception architecture using the cost sensitive loss functions proposed not only in \cite{Wang_IJCNN_2016} but also in \cite{Focal_loss:Lin_ICCV_2017} for the \textit{``All lights''} configuration using imbalanced data. We show the results for the newly trained models in the table below using the MCC metric which is known to be robust in the presence of imbalanced data. These results suggest random sampling to be better than using a loss function that penalizes mean false error \cite{Wang_IJCNN_2016} with imbalanced data. Also, there is no significant change in the MCC metric with the use of focal loss \cite{Focal_loss:Lin_ICCV_2017} with imbalanced data, indicating random under-sampling to be equally effective in our case. Moreover, it takes longer to train with imbalanced data as compared to random under-sampling.}
\begin{tabular}{|r|p{2.5cm}|p{2cm}|p{1.5cm}|}
    \hline
    & \textbf{Random under-sampling} & \textbf{Mean False Error \cite{Wang_IJCNN_2016}} & \textbf{Focal loss \cite{Focal_loss:Lin_ICCV_2017}}\\ \hline
    \textbf{MCC} & 0.7999 &  0.7514 & 0.8020 \\ \hline
\end{tabular}
\textcolor{blue}{We have now included the following lines in section \ref{subsubsec:data_balancing} for clarification.}
\changemarker{To avoid this problem, balancing the training data with random under-sampling has been considered as one of the effective, easy and widely accepted methods \cite{Buda_NN_2018}. Alternate approaches that use cost sensitive loss functions \cite{Wang_IJCNN_2016}, \cite{Focal_loss:Lin_ICCV_2017} with imbalanced training data did not show a significant change in the results in our case, but notably increased the training time. We have therefore adopted the former method and artificially balanced the patches extracted from every image by random undersampling, i.e.,\ we consider all the positive patches and randomly select an equal number of negative patches for balancing the dataset.}
\newline \newline 
\noindent \textbf{6.} \textit{It is unclear the definition of n(X) in pp. 4. Is this the number of patches? }
\newline
\noindent \textcolor{blue}{We apologies if this was not clear. ${n(X)}$ indicates the cardinality of the set ${X}$, where ${X}$ is a set of cracks represented by closed contours. To clarify this, we have now explicitly mentioned \changemarker{(${X}$ represents ${D, G}$ or any other set of cracks)}}.

\subsection{\textbf{Response to Comments of Reviewer \#2 (ID: 6299)}}

\noindent \textcolor{blue}{Below are the replies to the reviewer \#2's comments and the updates in the paper.}
\newline

\noindent \textbf{1.} \textit{``The paper is about developing a portable system for crack inspection.  Although there are no new methods presented, the paper shows some experimental results with various illumination changes.''}

\noindent \textcolor{blue}{We do not claim to propose a new architecture for detection in images. But as correctly pointed out, our novelty is in the proposed portable setup and a unique study that demonstrates the effects of lights placed at different heights on crack detection. Our work provides an insight about the illumination conditions that can help in improving crack detection in a challenging real-world industrial environment. We have added the following lines to the abstract to include this clarification.}
% \changemarker{\textit{More importantly, ours is the first of its kind of study that demonstrates how height-varying illumination conditions can affect crack detection with the use of existing state-of-the-art classifiers, in an attempt to provide an insight about the illumination conditions that can help in improving future techniques for crack detection.}}
\changemarker{More importantly, ours is the first a study that demonstrates how height-varying illumination conditions can affect crack detection with the use of existing state-of-the-art classifiers. We provide an insight about the illumination conditions that can help in improving crack detection in a challenging real-world industrial environment.}
